Super-Resolution with Deep Convolutional Sufficient Statistics

Inverse problems in image and audio, and super-resolution in particular, can be seen as high-dimensional structured prediction problems, where the goal is to characterize the conditional distribution of a high-resolution output given its low-resolution corrupted observation. When the scaling ratio is small, point estimates achieve impressive performance, but soon they suffer from the regression-to-the-mean problem, result of their inability to capture the multi-modality of this conditional distribution. Modeling high-dimensional image and audio distributions is a hard task, requiring both the ability to model complex geometrical structures and textured regions. In this paper, we propose to use as conditional model a Gibbs distribution, where its sufficient statistics are given by deep convolutional neural networks. The features computed by the network are stable to local deformation, and have reduced variance when the input is a stationary texture. These properties imply that the resulting sufficient statistics minimize the uncertainty of the target signals given the degraded observations, while being highly informative. The filters of the CNN are initialized by multiscale complex wavelets, and then we propose an algorithm to fine-tune them by estimating the gradient of the conditional log-likelihood, which bears some similarities with Generative Adversarial Networks. We evaluate experimentally the proposed approach in the image super-resolution task, but the approach is general and could be used in other challenging ill-posed problems such as audio bandwidth extension.

==> related.tex <==
\section{Solving inverse problems}
\label{inv_prob}

In this work, we use as case study two super-resolution problems, namely single-image super-resolution and
bandwidth extension of speech signals. This section briefly reviews the literature for these applications.

Single-image super resolution aims to construct a high-resolution (HR) image from a single low-resolution (LR) input. 
%
The goal is to characterize the conditional distribution of a HR output given its LR observation.
%
Most methods in the literature fall into two main categories: non-parametric and
parametric. The former aim to obtain the co-occurrence prior between the HR and LR local structures from an external
training database. The HR instance is produced by copying small patches from the most similar examples found in the training set (\cite{freeman2002example,sun2008image}).
%
Parametric models based on sparse coding models of image patches recieved a lot of attention, producing sucessful results (\cite{yang2008image}).
%
Recent works have shown that better results can be obtained 
when the models are tuned on recovery performance rather
than on data fitting (\cite{yang2012coupled}).
Coupled dictionaries, modeling HR and LR image patches respectively, are leaned such that the low and
high-resolution patch spaces relate via sparse representation.
%
Inspired by the great success achieved by
deep learning, \cite{dong2014learning} proposed to substitute the
sparse modeling stages with a CNN, reporting significantly impruvments over previously proposed models.
Following this effort, \cite{cui2014deep}  and \cite{wang2015self} explored ways of adapting the trained deep model to the given test image by exploiting self-similarities.
%
%Thanks to the end-to-end training and the large learning capacity were reported to  (\cite{dong2014learning}).





%When the scaling ratio is small, point estimates achieve impressive performance, but soon they suffer from the regression-to-the-mean problem, result of their inability to capture the multi-modality of this conditional distribution. 






